Mask-DPO: Generalizable Fine-grained Factuality Alignment of LLMs

Large language models (LLMs) exhibit hallucinations (i.e., unfaithful or nonsensical information) when serving as AI assistants in various domains. Since hallucinations always come with truthful content in the LLM responses, previous factuality alignment methods that conduct response-level preference learning inevitably introduced noises during training. Therefore, this paper proposes a fine-grained factuality alignment method based on Direct Preference Optimization (DPO), called Mask-DPO. Incorporating sentence-level factuality as mask signals, Mask-DPO only learns from factually correct sentences in the preferred samples and prevents the penalty on factual contents in the not preferred samples, which resolves the ambiguity in the preference learning. Extensive experimental results demonstrate that Mask-DPO can significantly improve the factuality of LLMs responses to questions from both in-domain and out-of-domain datasets, although these questions and their corresponding topics are unseen during training. Only trained on the ANAH train set, the score of Llama3.1-8B-Instruct on the ANAH test set is improved from 49.19% to 77.53%, even surpassing the score of Llama3.1-70B-Instruct (53.44%), while its FactScore on the out-of-domain Biography dataset is also improved from 30.29% to 39.39%. We further study the generalization property of Mask-DPO using different training sample scaling strategies and find that scaling the number of topics in the dataset is more effective than the number of questions. We provide a hypothesis of what factual alignment is doing with LLMs, on the implication of this phenomenon, and conduct proof-of-concept experiments to verify it. We hope the method and the findings pave the way for future research on scaling factuality alignment.

==> tables/ood.tex <==
\begin{wraptable}{r}{0.6\textwidth}
\centering
\small
\begin{tabular}{cccc}
\toprule
\textbf{Model} &\textbf{\# Correct} & \textbf{\# Incorrect} & \textbf{\% Score $\uparrow$} \\ \midrule
Qwen2-7B & 14.46 & 39.27 & 27.28 \\
Qwen2-72B & 20.13 & 40.09 & 34.06 \\
Gemma2-9B & 15.53 & 29.00 & 29.52 \\
Gemma2-27B & 19.27 & 36.59 & 29.99 \\
Yi1.5-6B & 10.84 & 59.65 & 15.81 \\
Yi1.5-9B & 10.63 & 62.67 & 15.33 \\
Yi1.5-34B & 17.01 & 52.76 & 25.49 \\
Llama3.1-8B & 16.83 & 31.57 & 30.29 \\
Llama3.1-70B & 23.58 & 31.59 & \textbf{40.47} \\ \midrule
FactTune & 15.93 & 23.97 & 37.97 \\ \midrule
\methodname{} & 12.16 & 15.24 & 39.39 \\ \bottomrule
\end{tabular}
\caption{\textbf{Evaluation results for the open-source models, FactTune, and our \methodname{} on out-of-domain data.} Here, we use the Biography dataset for evaluation.}
\label{tab: ood}
\end{wraptable}
